Redshift dependence of FRB host dispersion measures across cosmic epochs

We constrain the redshift dependence of (rest frame) host galaxy dispersion measures of localized Fast Radio Bursts (FRBs) by assuming it to vary as a simple power law ($\propto (1+z)^{\alpha}$). We simultaneously fit $\alpha$ as well as the host dispersion measure to the data of FRBs with known redshifts. We find that \color{black} $\alpha$ between 0 to 1 is preferred depending upon our modelling choices. Current data can constrain $|\alpha|\lesssim 2$ at a 68 percent confidence interval \color{black}. Such constraints have implications for our understanding of galaxy formation and can be used to inform galaxy and large scale simulations.

==> Befehle.tex <==
\newcommand{\beamav}[1]{\left< #1\right>}
\newcommand{\kDm}{k_{\rm D,m}}
\newcommand{\taudotc}{\tau'}
\newcommand{\zmuy}{{z_{\mu,y}}}
\newcommand{\nB}{n_{\rm m}}
\newcommand{\MJysr}{{\rm MJy\,sr^{-1}}}
\newcommand{\UnitInu}{{\rm W\,m^{-2}\,Hz^{-1}\,sr^{-1}}}
\newcommand{\Mpc}{{\rm Mpc}}
\newcommand{\GHz}{{\rm GHz}}
\newcommand{\kpc}{{\rm kpc}}
\newcommand{\pc}{{\rm pc}}
\newcommand{\lsup}[2]{ \ensuremath{{}^{#2}\!{#1}}}
\newcommand{\lsub}[2]{ \ensuremath{{}_{#2}\!{#1}}}
\newcommand{\lsim}{\lesssim}
\newcommand{\gsim}{\gtrsim}
\newcommand{\expf}[1]{{{\rm e}^{#1}}}
\newcommand{\Jbb}{\mathcal{J}}

%\newcommand{\ion}[2]{{\text{{\sc #1}\,{\sc #2}}}}
\newcommand{\transit}[3]{\rm #1^{\rm #2}#3\rightarrow\rm 1^{\rm 1}s}
\newcommand{\HeIlevel}[4]{{#1^{#2} {\rm #3}_{#4}}}   % \HeIlevel{n}{2S+1}{L}{J}
\newcommand{\mHe}{{m_{\rm He}}}
\newcommand{\Tz}{{T_{z}}}
\newcommand{\Tav}{{T_{\rm av}}}
\newcommand{\Tgs}{{T_{\gamma}^\ast}}
\newcommand{\TCMB}{T_{\rm CMB}}
\newcommand{\TRJ}{T_{\rm RJ}}
\newcommand{\Tgin}{{\Tg^{\rm in}}}
\newcommand{\tX}{{t_{\rm X}}}
\newcommand{\zX}{{z_{\rm X}}}
\newcommand{\zh}{{z_{\rm h}}}
\newcommand{\zmu}{{z_{\mu}}}
\newcommand{\zmudc}{{z_{\rm dc}}}
\newcommand{\zmubr}{{z_{\rm br}}}
\newcommand{\ye}{{y_{\rm e}}}
\newcommand{\yff}{{y_{\rm ff}}}
%\newcommand{\Thz}{{\theta_{z}}}
\newcommand{\sigmah}{{\sigma_{\rm h}}}
\newcommand{\xmat}{x_{\rm m}}

\newcommand{\xD}{{{x_{\rm D}}}}
\newcommand{\Erfc}{{\rm Erfc}}
\newcommand{\tauS}{{\tau_{\rm  S}}}
\newcommand{\zi}{{z_{\rm i}}}
\newcommand{\zs}{{z_{\rm s}}}
\newcommand{\ze}{{z_{\rm e}}}
\newcommand{\nbb}{{n^{\rm pl}}}
\newcommand{\nbbnu}{{n^{\rm pl}_\nu}}
\newcommand{\pdeath}{{p_{\rm d}}}
\newcommand{\pem}{{p_{\rm em}}}
\newcommand{\psc}{{p_{\rm sc}}}
\newcommand{\nL}{{n_{\rm L}}}
\newcommand{\tauHd}{\tau^{\rm H}_{\rm d}}
\newcommand{\tauDd}{\tau^{\rm D}_{\rm d}}

\newcommand{\omegab}{{\Omega_{\rm b}h^2}}
\newcommand{\omegadm}{{\Omega_{\rm dm}h^2}}
\newcommand{\omegak}{{\Omega_{\rm K}}}
\newcommand{\logAs}{\log(10^{9} A_{\rm S})}
\newcommand{\nS}{n_{\rm S}}
\newcommand{\nT}{n_{\rm T}}
\newcommand{\nrun}{n_{\rm run}}
\newcommand{\asz}{A_{\rm SZ}}
\newcommand{\YHe}{Y_{\rm p}}
\newcommand{\Nnu}{N_{\nu}}
\newcommand{\Planck}{{\sc Planck}}
\newcommand{\Ngpl}{N^{\rm Pl}_{\gamma}}

\newcommand{\zdc}{{{\rm few}\times 10^5}}
\newcommand{\nut}{{\tilde{\nu}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\gkin}{{\mathcal{Y}_{\rm kin}}}
\newcommand{\gkinh}{{\mathcal{\hat{Y}}_{\rm kin}}}
\newcommand{\gth}{{\mathcal{C}_{\rm th}}}
\newcommand{\gthh}{{\mathcal{\hat{C}}_{\rm th}}}

\newcommand{\Deltaprim}{{\Delta_{\rm pr}}}

\newcommand{\DeltaanRJ}{{\Delta_{\rm an}^{\rm RJ}}}
\newcommand{\Deltaanx}{{\hat{\Delta}_{\rm an}}}
\newcommand{\Deltaan}{{\Delta_{\rm an}}}

\newcommand{\vbetac}{{{\boldsymbol\beta}_{\rm c}}}
\newcommand{\vbetach}{{\hat{{\boldsymbol\beta}}_{\rm c}}}
\newcommand{\betac}{\beta_{\rm c}}
\newcommand{\betacpar}{{\beta_{\rm c,\parallel}}}
\newcommand{\betactr}{{\beta_{\rm c,\perp}}}
\newcommand{\betacsq}{{\beta^2_{\rm c}}}
\newcommand{\betacparsq}{{\beta^2_{\rm c,\parallel}}}
\newcommand{\betactrsq}{{\beta^2_{\rm c,\perp}}}
\newcommand{\muc}{\mu_{\rm c}}
\newcommand{\x}{{\hat{x}}}
\newcommand{\xem}{{x'_{\rm e}}}

\newcommand{\vbetao}{{{\boldsymbol\beta}_{\rm o}}}
\newcommand{\vbetaoh}{{\hat{{\boldsymbol\beta}}_{\rm o}}}
\newcommand{\betao}{\beta_{\rm o}}
\newcommand{\muo}{\mu_{\rm o}}

\newcommand{\vbetap}{{{\boldsymbol\beta}_{\rm p}}}
\newcommand{\vbetaph}{{\hat{{\boldsymbol\beta}}_{\rm p}}}
\newcommand{\betap}{\beta_{\rm p}}

\newcommand{\vecJ}[1]{{\bf #1}}
\newcommand{\vecx}{{\vecJ{x}}}
\newcommand{\vecxc}{{\vecJ{x}_{\rm c}}}
\newcommand{\vk}{{\vecJ{k}}}
\newcommand{\vkp}{{\vecJ{k'}}}
\newcommand{\vkh}{{\vecJ{\hat{k}}}}
\newcommand{\vkhp}{{\vecJ{\hat{k}'}}}

\newcommand{\gh}{{\hat{\gamma}}}
\newcommand{\vg}{{\vecJ{\boldsymbol\gamma}}}
\newcommand{\vgh}{{\hat{\boldsymbol\gamma}}}
\newcommand{\vghp}{{\hat{\boldsymbol\gamma}'}}

\newcommand{\kproj}[1]{{ \{#1\} }}
\newcommand{\gproj}[1]{{ [#1] }}


\newcommand{\vb}{{\boldsymbol{\beta}}}
\newcommand{\vbh}{{\boldsymbol{\hat{\beta}}}}

\newcommand{\vbc}{{\boldsymbol{\beta}_{\rm p}}}
\newcommand{\vbch}{{\boldsymbol{\hat{\beta}}_{\rm p}}}
\newcommand{\gammac}{{\gamma_{\rm p}}}

\newcommand{\NP}{{n(\xe, \vkh)}}
\newcommand{\NPP}{{n(\xe, \vkhp)}}

\newcommand{\vp}{{\vecJ{p}}}
\newcommand{\vpp}{{\vecJ{p'}}}
\newcommand{\vph}{{\vecJ{\hat{p}}}}
\newcommand{\vpph}{{\vecJ{\hat{p}'}}}

\newcommand{\mus}{{\mu_{\rm s}}}
\newcommand{\mue}{{\mu_{\rm e}}}
\newcommand{\muC}{{\mu_{\rm c}}}
\newcommand{\muCp}{{\mu'_{\rm c}}}

\newcommand{\phis}{{\phi_{\rm s}}}
\newcommand{\phic}{{\phi_{\rm p}}}

\newcommand{\Deltae}{\Delta_{\rm e}}
\newcommand{\Deltaxe}{\Delta \xe}
\newcommand{\Deltaye}{\Delta y_{\rm e}}
\newcommand{\Deltaze}{\Delta z_{\rm e}}

%\newcommand{\xg}{x_{\gamma}}
\newcommand{\xg}{x}
\newcommand{\xav}{x_{\rm av}}
\newcommand{\xgc}{x_{\rm c}}

\newcommand{\Theav}{\theta_{\rm e, av}}
\newcommand{\Teav}{T_{\rm e, av}}
\newcommand{\Thez}{\theta_{z}}
\newcommand{\taudot}{\dot{\tau}}
\newcommand{\kD}{k_{\rm D}}
\newcommand{\rs}{r_{\rm s}}
\newcommand{\cs}{c_{\rm s}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%\newcommand{\twosav}[1]{{\left<\,#1\,\right>^{\rm 2\gamma}_{\rm  2s}}}
\newcommand{\twosav}[1]{{\left<\,#1\,\right>^{2\gamma}_{\rm 2s}}}
\newcommand{\twopav}[1]{{\left<\,#1\,\right>_{\rm Ly-\alpha}}}
\newcommand{\twosavg}[3]{{\left<\,#1\,\right>^{#2}_{#3}}}

\newcommand{\Op}[1]{\hat{\bf #1}}

\newcommand{\nmi}{n_{-}}

\newcommand{\npl}{n_{+}}

\newcommand{\ngamma}{n_\gamma}

\newcommand{\vrel}{|v_{\rm rel}|}

\newcommand{\xt}{\tilde{x}}

\newcommand{\xe}{x_{\rm e}}

\newcommand{\xc}{x_{\rm c}}



\newcommand{\Absatz}{\vspace{2ex}}

\newcommand{\id}{{\,\rm d}}



\newcommand{\beq}{\begin{equation}}   %

\newcommand{\eeq}{\end{equation}}   %

\newcommand{\vc}[1]{\ensuremath{\mathbf{#1}}}

\newcommand{\Div}[1]{\vek{\nabla} \! \cdot \vek{#1}}   %

\newcommand{\Rot}[1]{\vek{\nabla} \times \vek{#1}}



\newcommand{\beqa}{\begin{eqnarray}}   %

\newcommand{\eeqa}{\end{eqnarray}}   %

\newcommand{\beal}{\begin{align}}

\newcommand{\enal}{\end{align}}

\newcommand{\bspl}{\begin{split}}

\newcommand{\espl}{\end{split}}

\newcommand{\bsub}{\begin{subequations}}

\newcommand{\esub}{\end{subequations}}

\newcommand{\bmulti}{\begin{multline}}   %

\newcommand{\beqm}{\begin{mathletters}}   %

\newcommand{\eeqm}{\end{mathletters}}   %



\newcommand{\Doll}[1]{\bf#1\rm}

\newcommand{\Glossar}[2]{\bf#1 \rm\quad #2}

\newcommand{\Abkuerz}[1]{#1}

\newcommand{\Abschnitt}[1]{\subsection*{#1}}

\newcommand{\Abst}[1]{\,#1}



\newcommand{\kB}{k_{\rm B}}

\newcommand{\me}{m_{\rm e}}

\newcommand{\Ne}{N_{\rm e}}

\newcommand{\Np}{n_{\rm p}}

\newcommand{\Nb}{n_{\rm b}}

\newcommand{\Te}{T_{\rm e}}

\newcommand{\Tg}{T_{\gamma}}

\newcommand{\The}{\theta_{\rm e}}

\newcommand{\Thg}{\theta_{\gamma}}

\newcommand{\mprot}{m_{\rm p}}

\newcommand{\sigT}{\sigma_{\rm T}}

\newcommand{\sigKN}{\sigma_{\rm K-N}}

\newcommand{\rC}{r_{\rm c}}



\newcommand{\nPl}{n_{\rm Pl}}

\newcommand{\nBE}{n_{\rm BE}}

\newcommand{\nW}{n_{\rm W}}

\newcommand{\rhoPl}{\rho_{\rm Pl}}

\newcommand{\rhoBE}{\rho_{\rm BE}}

\newcommand{\NPl}{N_{\rm Pl}}

\newcommand{\NBE}{N_{\rm BE}}



\newcommand{\vek} [1]{\mbox{\boldmath${#1}$\unboldmath}}

\newcommand{\matr} [1]{\mbox{$\hat{#1}$}}

\newcommand{\SP}[2]{\mbox{$\vek{#1}\cdot\vek{#2}$}}

\newcommand{\pd}{\partial}

\newcommand{\pAb}[2]{\frac{\displaystyle\pd #1}{\displaystyle\pd #2}}
\newcommand{\pAbc}[3]{\left.\frac{\displaystyle\pd #1}{\displaystyle\pd #2}\right|_{#3}}

\newcommand{\PAb}[3]{\frac{\displaystyle\pd^{#3} #1}{\displaystyle\pd {#2}^{#3}}}

\newcommand{\tAb}[2]{\frac{\displaystyle d #1}{\displaystyle d #2}}

\newcommand{\TAb}[3]{\frac{\displaystyle d^{#3} #1}{\displaystyle d {#2}^{#3}}}

\newcommand{\Abl}[2]{\frac{{\rm d} #1}{{\rm d} #2}}

\newcommand{\AKc}[1]{{\rm C}_{#1}}

\newcommand{\AKs}[1]{{\rm S}_{#1}}

\newcommand{\sgn}[1]{\,{\rm sgn}\,{#1}}

\newcommand{\Mitw}[1]{\left<#1\right>}



\newcommand{\Vv}[1]{\mbox{${#1}$}}

\newcommand{\Vvek}[2]{\mbox{${#1}^{#2}$}}

\newcommand{\VvN}[1]{\mbox{${#1}_{0}$}}

\newcommand{\VvNN}[1]{\mbox{${#1}_{0}^2$}}

\newcommand{\VSP}[2]{\mbox{$\Vv{#1}\Vv{#2}$}}



\newcommand{\STV}[1]{\mbox{$\tilde{#1}$}}



%\renewcommand{\eqref}[1]{(\ref{#1})}

\newcommand{\figref}[1]{Abb.\ref{#1}}

\newcommand{\tabref}[1]{Tab.\ref{#1}}

\newcommand{\kapref}[1]{Kap.\ref{#1}}

\newcommand{\deltaD}[1]{\mbox{$\delta( {#1} )$}}

\newcommand{\Aut}[1]{\it{#1}\rm }

\newcommand{\AutP}[1]{\it{#1}\rm }

\newcommand{\AutPet}[1]{\it{#1 et al.}\rm }

\newcommand{\AutPno}[1]{{#1}\rm }

\newcommand{\AutPnoet}[1]{{#1 et al.}\rm }



\newcommand{\Vvekm}[1]{\mbox{$\Vvek{#1}{\mu}$}}

\newcommand{\Vvekcv}[2]{\mbox{${#1}_{#2}$}}

\newcommand{\Vvekcvm}[1]{\mbox{$\Vvekcv{#1}{\mu}$}}



\newcommand{\pot}[2]{#1 \times 10^{#2}}
\newcommand{\poterr}[3]{(#1\pm#2)\times10^{#3}}


\newcommand{\ngam}{n_{\gamma}}



% Cosmology

\newcommand{\tC}{t_{\rm C}}

\newcommand{\tK}{t_{\rm K}}

\newcommand{\tge}{t_{\gamma \rm e}}

\newcommand{\teg}{t_{\rm e\gamma}}

\newcommand{\texp}{t_{\rm exp}}

\newcommand{\ThCMB}{\Theta_{2.7}}
\newcommand{\Thz}{\theta_{z}}
\newcommand{\Yp}{Y_{\rm p}}

\newcommand{\Obhh}{\Omega_{\rm b}h^2}

\newcommand{\Omhh}{\Omega_{\rm m}h^2}

\newcommand{\zeq}{z_{\rm eq}}
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 

